New theoretical Period-Luminosity-Metallicity relations for RR Lyrae in the Rubin-LSST filters

The revolutionary power of future Rubin-LSST observations will allow us to significantly improve the physics of pulsating stars, including RR Lyrae. In this context, an updated theoretical scenario predicting all the relevant pulsation observables in the corresponding photometric filters is mandatory. The bolometric light curves based on a recently computed extensive set of nonlinear convective pulsation models for RR Lyrae stars, covering a broad range in metal content and transformed into the Rubin-LSST photometric system. Predicted Rubin-LSST mean magnitudes and pulsation amplitudes have been adopted to built the Bailey diagrams (luminosity amplitude vs period) and the color-color diagrams in these bands. The current findings indicate that the gLSST-rLSST, rLSST-iLSST colors obey to a well defined linear relation with the metal content. Moreover, the Period Luminosity relations display in the reddest filters (rLSST,iLSST,zLSST,yLSST) a significant dependence on the assumed metal abundance. In particular, more metal-rich RR Lyrae are predicted to be fainter at fixed period. Metal-dependent Period-Wesenheit relations for different combinations of optical and NIR filters are also provided. These represent powerful tools to infer individual distances independently of reddening uncertainties, once the metal abundance is known and no relevant deviations from the adopted extinction law occur. Finally, we also derived new linear and quadratic absolute magnitude metallicity relations (gLSST vs [Fe/H]) and the metallicity coefficient is consistent with previous findings concerning the B and the V band.

==> ColorColoZ.Fit_dydz_standard_rizY_gFeH_AB_2MassLevels_final.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Fri May  6 15:26:00 2022
\begin{table*}
\centering
\begin{tabular}{ccccccc}
  \hline
Col1 & Col2 & $\alpha$ & $\beta$ & $\gamma$ & $\sigma$ & $R^2$\\ 
  \hline
    \hline
    \multicolumn{7}{c}{$Col_2=\alpha \cdot Col_1 +\beta [Fe/H] +\gamma$} \\
   $(g-r)_{LSST}$ & $(r-i)_{LSST}$ & $0.562 \pm 0.006$ & $-0.0215 \pm 0.0007$ & $-0.1089 \pm 0.0013$ & 0.008 & 0.97\\ 
   $(r-i)_{LSST}$ & $(g-r)_{LSST}$ & $1.73 \pm 0.02$ & $0.0381 \pm 0.0012$ & $0.193 \pm 0.002$ & 0.013 & 0.98 \\ 
    \hline
    \hline
    \multicolumn{7}{c}{$[Fe/H]=\alpha \cdot Col_1 +\beta \cdot Col_2 +\gamma$} \\
   $(g-r)_{LSST}$ & $(r-i)_{LSST}$ & $21.4 \pm 0.6$ & $-37 \pm 1$ & $-4.36 \pm 0.1$ & 0.313 & 0.82 \\ 
   \hline
\end{tabular}
\caption{This table contains the fitting results for color-color-[FeH] relations. Columns 1 and 2 contain the fitted colors, while the coefficients of the obtained relations are reported in columns 3-5. Finally, columns 6 and 7 contain the rms of the residuals around the fit and the coefficient of determination, respectively.} 
\label{tab-ColColZFit}
\end{table*}


==> PLFeH_coeffs_dydz_standard_rizY_gFeH_AB_2MassLevels_final.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Wed May  4 23:45:47 2022
\begin{table*}
\centering
\begin{tabular}{lcccccccc}
  \hline
Mode & N & Band$_{LSST}$ & $R^2$ & $\sigma$ & $\alpha$ & $\beta$ & $\gamma$ & $\delta$\\ \hline
  \hline
    \multicolumn{9}{c}{$Mag=\alpha+\beta{\log{P}}+\gamma[Fe/H]$} \\
F & 155 & $r$ & 0.750 & 0.128 & $0.25 \pm 0.02$ & $-1.35 \pm 0.08$ & $0.163 \pm 0.014$ & - \\
  FO & 93 & $r$ & 0.916 & 0.075 & $-0.19 \pm 0.03$ & $-1.66 \pm 0.06$ & $0.149 \pm 0.011$ & -\\ 
  FO (F slope) & 93 & $r$ & 0.650 & 0.084 & $-0.07 \pm 0.02$ & $-1.35 \pm 0.09$ & $0.156 \pm 0.012$ & -\\ 
  F+FO  & 248 & $r$ & 0.733 & 0.132 & $0.22 \pm 0.02$ & $-1.25 \pm 0.06$ & $0.168 \pm 0.012$ & - \\ 
  F & 155 & $i$ & 0.863 & 0.099 & $0.21 \pm 0.02$ & $-1.6 \pm 0.07$ & $0.163 \pm 0.011$ & -\\ 
  FO & 93 & $i$ & 0.955 & 0.059 & $-0.22 \pm 0.02$ & $-1.87 \pm 0.05$ & $0.149 \pm 0.008$ & -\\ 
  FO (F slope) & 93 & $i$ & 0.738 & 0.067 & $-0.12 \pm 0.014$ & $-1.6 \pm 0.07$ & $0.154 \pm 0.01$ & -\\ 
  F+FO  & 248 & $i$ & 0.850 & 0.105 & $0.18 \pm 0.02$ & $-1.52 \pm 0.05$ & $0.166 \pm 0.009$ & -\\ 
  F & 155 & $z$ & 0.903 & 0.087 & $0.23 \pm 0.02$ & $-1.73 \pm 0.06$ & $0.168 \pm 0.01$ & -\\ 
  FO & 93 & $z$ & 0.968 & 0.052 & $-0.21 \pm 0.02$ & $-1.99 \pm 0.04$ & $0.152 \pm 0.008$ & -\\ 
  FO (F slope) & 93 & $z$ & 0.780 & 0.061 & $-0.104 \pm 0.013$ & $-1.73 \pm 0.06$ & $0.158 \pm 0.009$ & -\\ 
  F+FO  & 248 & $z$ & 0.893 & 0.092 & $0.205 \pm 0.014$ & $-1.67 \pm 0.04$ & $0.17 \pm 0.008$ & -\\ 
  F & 155 & $y$ & 0.905 & 0.086 & $0.23 \pm 0.02$ & $-1.75 \pm 0.06$ & $0.167 \pm 0.01$ & -\\ 
  FO & 93 & $y$ & 0.967 & 0.053 & $-0.2 \pm 0.02$ & $-2 \pm 0.04$ & $0.151 \pm 0.008$ & -\\ 
  FO (F slope) & 93 & $y$ & 0.782 & 0.061 & $-0.109 \pm 0.013$ & $-1.75 \pm 0.06$ & $0.157 \pm 0.009$ & -\\ 
  F+FO  & 248 & $y$ & 0.896 & 0.092 & $0.204 \pm 0.014$ & $-1.68 \pm 0.04$ & $0.169 \pm 0.008$ & -\\ 
      \hline
  \hline
    \multicolumn{9}{c}{$W=\alpha+\beta{\log{P}}+\gamma[Fe/H]$} \\
  F & 155 & $g,u-g$ & 0.468 & 0.219 & $-3.28 \pm 0.04$ & $-1.29 \pm 0.14$ & $-0.22 \pm 0.02$ & -\\ 
  FO & 93 & $g,u-g$ & 0.593 & 0.145 & $-3.58 \pm 0.06$ & $-1.33 \pm 0.12$ & $-0.1 \pm 0.02$ & -\\ 
  FO (F slope) & 93 & $g,u-g$ & 0.219 & 0.144 & $-3.56 \pm 0.03$ & $-1.29 \pm 0.14$ & $-0.1 \pm 0.02$ & -\\ 
  F+FO & 248 & $g,u-g$ & 0.326 & 0.229 & $-3.25 \pm 0.04$ & $-0.94 \pm 0.11$ & $-0.16 \pm 0.02$ & -\\ 
  F   &         155 & $r,u-r$ &   0.869 & 0.010  &  $-1.622\pm 0.019$ & $-2.09\pm  0.07$ & $-0.059\pm   0.011$     &      -  \\     
  FO   &          93 & $r,u-r$ &   0.926 & 0.073  &  $-1.95\pm 0.03$ & $-2.07\pm  0.06$ & $-0.010\pm   0.010$     &      -   \\         
  FO (F slope) &  93 & $r,u-r$ &   0.011 & 0.073  &  $-1.960\pm 0.015$ & $-2.09\pm  0.07$ & $-0.011\pm   0.010$     &      -   \\         
  F+FO     &     248 & $r,u-r$ &   0.841 & 0.109  &  $-1.606\pm 0.017$ & $-1.89\pm  0.05$ & $-0.031\pm   0.010$     &      - \\         
  F & 155 & $r,g-r$ & 0.961 & 0.068 & $-0.489 \pm 0.013$ & $-2.63 \pm 0.04$ & $0.047 \pm 0.008$ & -\\ 
  FO & 93 & $r,g-r$ & 0.980 & 0.048 & $-0.85 \pm 0.02$ & $-2.58 \pm 0.04$ & $0.054 \pm 0.007$ & -\\ 
  FO (F slope) & 93 & $r,g-r$ & 0.399 & 0.048 & $-0.867 \pm 0.01$ & $-2.63 \pm 0.04$ & $0.053 \pm 0.007$ & -\\ 
  F+FO & 248 & $r,g-r$ & 0.967 & 0.064 & $-0.486 \pm 0.01$ & $-2.54 \pm 0.03$ & $0.053 \pm 0.006$ & -\\ 
  F & 155 & $i,g-i$ & 0.982 & 0.046 & $-0.178 \pm 0.009$ & $-2.51 \pm 0.03$ & $0.11 \pm 0.005$ & -\\ 
  FO & 93 & $i,g-i$ & 0.990 & 0.035 & $-0.565 \pm 0.013$ & $-2.56 \pm 0.03$ & $0.104 \pm 0.005$ & -\\ 
  FO (F slope) & 93 & $i,g-i$ & 0.830 & 0.035 & $-0.546 \pm 0.007$ & $-2.51 \pm 0.03$ & $0.105 \pm 0.005$ & -\\ 
  F+FO & 248 & $i,g-i$ & 0.983 & 0.046 & $-0.186 \pm 0.007$ & $-2.47 \pm 0.02$ & $0.111 \pm 0.004$ & - \\ 
  F & 155 & $z,i-z$ & 0.975 & 0.051 & $0.295 \pm 0.01$ & $-2.13 \pm 0.03$ & $0.185 \pm 0.006$ & -\\ 
  FO & 93 & $z,i-z$ & 0.990 & 0.033 & $-0.146 \pm 0.013$ & $-2.38 \pm 0.03$ & $0.164 \pm 0.005$ & -\\ 
  FO (F slope) & 93 & $z,i-z$ & 0.884 & 0.045 & $-0.052 \pm 0.009$ & $-2.13 \pm 0.03$ & $0.169 \pm 0.006$ & -\\ 
  F+FO & 248 & $z,i-z$ & 0.972 & 0.056 & $0.269 \pm 0.009$ & $-2.14 \pm 0.03$ & $0.181 \pm 0.005$ & -\\ 
  F & 155 & $y,g-y$ & 0.983 & 0.042 & $0.071 \pm 0.008$ & $-2.23 \pm 0.03$ & $0.147 \pm 0.005$ & -\\ 
  FO & 93 & $y,g-y$ & 0.990 & 0.032 & $-0.341 \pm 0.013$ & $-2.37 \pm 0.03$ & $0.134 \pm 0.005$ & -\\ 
  FO (F slope) & 93 & $y,g-y$ & 0.883 & 0.037 & $-0.288 \pm 0.008$ & $-2.23 \pm 0.03$ & $0.136 \pm 0.005$ & -\\ 
  F+FO & 248 & $y,g-y$ & 0.977 & 0.050 & $0.054 \pm 0.008$ & $-2.19 \pm 0.02$ & $0.147 \pm 0.004$ & - \\ 
      \hline
  \hline
     \multicolumn{9}{c}{$Mg=\alpha+\gamma[Fe/H]+\delta[Fe/H]^2$} \\
F+FO  & 248 & $g,[Fe/H]$ & 0.384 & 0.209 & $0.62 \pm 0.03$ & $0 \pm 0$ & $0.23 \pm 0.02$ & -\\ 
  F+FO  & 248 & $g,[Fe/H]^2$  & 0.396 & 0.208 & $0.67 \pm 0.03$ & $0 \pm 0$ & $0.36 \pm 0.06$ & $0.06 \pm 0.03$\\ 
   \hline
\end{tabular}
\caption{The coefficients of the fitted PLZ ($Mag = \alpha + \beta\log P + \gamma [FeH]$), PWZ ($W = \alpha + \beta\log P + \gamma [FeH]$) and absolute G magnitude versus [Fe/H] (in both the linear $M_g = \alpha  + \gamma[FeH]$ and the quadratic $M_g = \alpha  + \gamma[FeH] +\delta{[Fe/H]^2}$ form). The following quantities are listed: (column 1) the mode of the fitted sources; (column 2) the number of models used in the fit;
(column 3) the photometric band; (column 4) the coefficient of determination $R^2$; (column 5) the rms of residuals around the fitted relation; (columns 6-9) the parameters of the different fitted relations.} 
\label{tab-plzCoeffs}
\end{table*}


==> mainParameters.lsst.FO_dydz_standard_rizY_gFeH_AB_2MassLevels.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Feb 28 13:01:10 2022
\begin{table*}
\centering
\tabcolsep=0.11cm
\begin{tabular}{cccccccccccccccccc}
  \hline
Z & Y & P & M & $\log(L/L_\odot)$ & $T_{eff}$ & $ \langle u_{LSST} \rangle$ & A$_u$ & $ \langle g_{LSST} \rangle$ & A$_g$ & $ \langle r_{LSST} \rangle$ & A$_r$ & $ \langle i_{LSST} \rangle$ & A$_i$ & $ \langle z_{LSST} \rangle$ & A$_z$ & $ \langle y_{LSST} \rangle$ & A$_y$ \\  
(dex) & (dex) & (days) & ($M_\odot$) & (dex) & (K) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) \\  
  \hline
0.0001 & 0.245 & 0.4107 & 0.80 & 1.760 & 6600 & 1.301 & 0.607 & 0.346 & 0.710 & 0.243 & 0.528 & 0.255 & 0.411 & 0.297 & 0.354 & 0.304 & 0.356 \\ 
  0.0001 & 0.245 & 0.3910 & 0.80 & 1.760 & 6700 & 1.292 & 0.756 & 0.327 & 0.873 & 0.246 & 0.665 & 0.272 & 0.532 & 0.319 & 0.472 & 0.325 & 0.477 \\ 
  0.0001 & 0.245 & 0.3721 & 0.80 & 1.760 & 6800 & 1.282 & 0.962 & 0.310 & 1.090 & 0.254 & 0.805 & 0.293 & 0.630 & 0.345 & 0.558 & 0.351 & 0.568 \\ 
  0.0001 & 0.245 & 0.3553 & 0.80 & 1.760 & 6900 & 1.272 & 1.111 & 0.297 & 1.214 & 0.264 & 0.885 & 0.315 & 0.685 & 0.373 & 0.607 & 0.379 & 0.618 \\ 
  0.0001 & 0.245 & 0.3386 & 0.80 & 1.760 & 7000 & 1.263 & 1.133 & 0.286 & 1.212 & 0.273 & 0.880 & 0.337 & 0.680 & 0.400 & 0.605 & 0.406 & 0.615 \\ 
  0.0001 & 0.245 & 0.3235 & 0.80 & 1.760 & 7100 & 1.255 & 1.096 & 0.274 & 1.162 & 0.280 & 0.834 & 0.355 & 0.639 & 0.425 & 0.570 & 0.430 & 0.580 \\ 
   \hline
\end{tabular}
\caption{First overtone model parameters: the values of Z and Y are listed in columns 1 and 2, respectively, 
the period of pulsation is in column 3, the mass, luminosity and effective temperatures are listed 
in columns 4, 5, and 6, while the LSST light curve intensity average magnitudes and amplitudes are reported in the columns 
from 7 to 18 for all the selected bands. The complete table is available in electronic format.} 
\label{tab-mainParameters-FO}
\end{table*}


==> mainParameters.lsst.F_dydz_standard_rizY_gFeH_AB_2MassLevels.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Feb 28 12:52:24 2022
\begin{table*}
\centering
\tabcolsep=0.11cm
\begin{tabular}{cccccccccccccccccc}
  \hline
Z & Y & P & M & $\log(L/L_\odot)$ & $T_{eff}$ & $ \langle u_{LSST} \rangle$ & A$_u$ & $ \langle g_{LSST} \rangle$ & A$_g$ & $ \langle r_{LSST} \rangle$ & A$_r$ & $ \langle i_{LSST} \rangle$ & A$_i$ & $ \langle z_{LSST} \rangle$ & A$_z$ & $ \langle y_{LSST} \rangle$ & A$_y$ \\  
(dex) & (dex) & (days) & ($M_\odot$) & (dex) & (K) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) \\  
  \hline
0.0001 & 0.245 & 0.7624 & 0.80 & 1.760 & 6000 & 1.375 & 0.335 & 0.461 & 0.379 & 0.245 & 0.274 & 0.187 & 0.212 & 0.189 & 0.179 & 0.191 & 0.173 \\ 
  0.0001 & 0.245 & 0.7210 & 0.80 & 1.760 & 6100 & 1.366 & 0.654 & 0.445 & 0.752 & 0.245 & 0.559 & 0.196 & 0.438 & 0.203 & 0.375 & 0.205 & 0.369 \\ 
  0.0001 & 0.245 & 0.6839 & 0.80 & 1.760 & 6200 & 1.354 & 0.833 & 0.426 & 0.958 & 0.244 & 0.725 & 0.206 & 0.575 & 0.219 & 0.502 & 0.222 & 0.501 \\ 
  0.0001 & 0.245 & 0.6469 & 0.80 & 1.760 & 6300 & 1.343 & 0.879 & 0.407 & 1.013 & 0.245 & 0.765 & 0.219 & 0.607 & 0.238 & 0.531 & 0.241 & 0.532 \\ 
  0.0001 & 0.245 & 0.6133 & 0.80 & 1.760 & 6400 & 1.330 & 0.932 & 0.385 & 1.067 & 0.247 & 0.822 & 0.234 & 0.669 & 0.259 & 0.597 & 0.263 & 0.600 \\ 
  0.0001 & 0.245 & 0.5810 & 0.80 & 1.760 & 6500 & 1.315 & 1.184 & 0.362 & 1.336 & 0.250 & 1.002 & 0.253 & 0.797 & 0.284 & 0.710 & 0.288 & 0.718 \\ 
   \hline
\end{tabular}
\caption{Fundamental model parameters: the values of Z and Y are listed in columns 1 and 2, respectively, 
the period of pulsation is in column 3, the mass, luminosity and effective temperatures are listed 
in columns 4, 5, and 6, while the LSST light curve intensity average magnitudes and amplitudes are reported in the columns 
from 7 to 18 for all the selected bands. The complete table is available in electronic format.} 
\label{tab-mainParameters-F}
\end{table*}


==> mainParameters.lsst.ZYML_dydz_standard_rizY_gFeH_AB_2MassLevels.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Wed Mar  9 23:31:45 2022
\begin{table}
\centering
\tabcolsep=0.11cm
\begin{tabular}{lcccc}
  \hline
$Z$ & $Y$ & $M$ & $\log(L/L_\odot)$ &  \\ 
$(dex)$ & $(dex)$ & $(M_\odot)$ & $(dex)$ &\\
  \hline
0.0001 & 0.245 & 0.800 & 1.76 & ZAHB \\ 
  0.0001 & 0.245 & 0.800 & 1.86 & Brighter \\ 
  0.0001 & 0.245 & 0.720 & 1.96 & Evolved \\ 
  0.0003 & 0.245 & 0.716 & 1.72 & ZAHB \\ 
  0.0003 & 0.245 & 0.716 & 1.82 & Brighter \\ 
  0.0003 & 0.245 & 0.650 & 1.92 & Evolved \\ 
  0.0006 & 0.245 & 0.670 & 1.69 & ZAHB \\ 
  0.0006 & 0.245 & 0.670 & 1.79 & Brighter \\ 
  0.0006 & 0.245 & 0.600 & 1.89 & Evolved \\ 
  0.0010 & 0.245 & 0.640 & 1.67 & ZAHB \\ 
  0.0010 & 0.245 & 0.640 & 1.77 & Brighter \\ 
  0.0010 & 0.245 & 0.580 & 1.87 & Evolved \\ 
  0.0040 & 0.250 & 0.590 & 1.61 & ZAHB \\ 
  0.0040 & 0.250 & 0.590 & 1.71 & Brighter \\ 
  0.0040 & 0.250 & 0.530 & 1.81 & Evolved \\ 
  0.0080 & 0.256 & 0.570 & 1.58 & ZAHB \\ 
  0.0080 & 0.256 & 0.570 & 1.68 & Brighter \\ 
  0.0080 & 0.256 & 0.510 & 1.78 & Evolved \\ 
  0.0200 & 0.270 & 0.540 & 1.49 & ZAHB \\ 
  0.0200 & 0.270 & 0.540 & 1.59 & Brighter \\ 
  0.0200 & 0.270 & 0.510 & 1.69 & Evolved \\ 
   \hline
\end{tabular}
\caption{This table contains the elemental abundance Z and the Helium abundance Y of the considered models, respectively
in the column 1 and 2, the mass M and the luminosity $\log L/L_\odot$ respectively in the columns 3 and 4, while in the column 5 a 
string tag is contained labeling the ZAHB, the Brighter and the Evolved models introduced in the text.} 
\label{tab-main-ZYML-params}
\end{table}

